Stabilizer formalism in linear optics and application to Bell-state discrimination

We propose a framework to analyze linear optical circuits based on an analogy with stabilizer formalism in quantum circuits, which provides efficiently computable formulas related to state discriminations. Hence, we analyze a Bell-state discrimination scheme with linear optics and ancillary single photons. With an increasing number of ancilla photons, the success probability of Bell-state discrimination has a maximum of $\frac{403}{512} \simeq 0.787$ at $28$ ancilla photons. By contrast, the corresponding two-qubit measurement asymptotically approaches a maximally entangling measurement.

==> perm_bell_aux.tex <==



==> perm_bell_sup_aux.tex <==


